Multi-Principal Assistance Games

Assistance games (also known as cooperative inverse reinforcement learning games) have been proposed as a model for beneficial AI, wherein a robotic agent must act on behalf of a human principal but is initially uncertain about the humans payoff function. This paper studies multi-principal assistance games, which cover the more general case in which the robot acts on behalf of N humans who may have widely differing payoffs. Impossibility theorems in social choice theory and voting theory can be applied to such games, suggesting that strategic behavior by the human principals may complicate the robots task in learning their payoffs. We analyze in particular a bandit apprentice game in which the humans act first to demonstrate their individual preferences for the arms and then the robot acts to maximize the sum of human payoffs. We explore the extent to which the cost of choosing suboptimal arms reduces the incentive to mislead, a form of natural mechanism design. In this context we propose a social choice method that uses shared control of a system to combine preference inference with social welfare optimization.

==> mpalg.tex <==
\subsection{Inducing Honest Human Strategies}

Optimal strategy for the learning phase is more complex. Each human principal is interested in maximizing their own utility. However, their actions in the learning phase not only directly provide utility, but also influence how the AI acts in the deployment phase. 

We consider how human $i$ optimally acts, given how other humans acts.
\begin{definition}[Best Response]
Given AI mechanism $\mathcal{M}$ and $\alpha$, define the best response of human $i$ to $\pi_{-i}$ as
\begin{equation}
    Br_i(\pi_{-i}, \mathcal{M}, \alpha) = \text{\normalfont argmax}_{\pi_i} U_i(\pi_i,\pi_{-i}, \mathcal{M}, \alpha),
\end{equation}
\end{definition}

Furthermore, we define the policy that maximizes reward in the original MDP.
\begin{definition}[Expert Policy]
Define the expert policy as \begin{equation}
    \pi^*_i = \text{\normalfont argmax}_{\pi_i} V(\pi_i, R_i)
\end{equation}
\end{definition}
The expert policy maximizes the reward from a single instance of the MDP, although it may be suboptimal for the two-stage game we constructed. These policies for a benchmark against which we can compare other policies. 

Ideally, the two-phase game would proceed as follows: in the learning phase, each human acts according to the expert policy while the AI learns each human's preferences; in the deployment phase, the AI acts to maximize the sum of these preferences. This is the assumption generally in inverse reinforcement learning situations. However, as seen before, humans may be incentivized to misrepresent these preferences by playing different policies in the learning phase. These policies may decreases social welfare relative to the expert policy in the deployment phase.

\begin{definition} [Dishonest Policies]
for human $i$, policy $\pi_i$ is dishonest if
\begin{equation}
    \sum_j \bE_P [U_j^D(\pi_i^*, \pi_{-i}^*, \mathcal{M}^*)] > \sum_j \bE_P[U_j^D(\pi_i, \pi_{-i}^*, \mathcal{M}^*)].
\end{equation}
\end{definition}  
In particular, we are interested in cases where dishonest policies may be the best response or yield greater utility than the expert policy to human $i$. Acting according the these policies would yield demonstrations that do not reflect the human's true reward function, but yield greater utility over the two phases.

With these definitions, we can analyze optimal human behavior for each individual. In the first case, we consider the optimal strategy if when the human's utility is weighted entirely to the learning phase, i.e. $\alpha = 1$. In this case, the dominant strategy is the expert policy. Each human maximizes their own utility by providing truthful demonstrations.
\begin{theorem}
$Br_i(\pi_{-i},\mathcal{M}, 1) = \pi^*_i$ for all $\pi_{-i},\mathcal{M}$.
\end{theorem}
\iffalse\begin{proof}
Since $\alpha = 1$, the entirety of utility of the human is determined by .
\begin{align*}
Br_i(\pi_{-i}) &= \text{argmax}_{\pi_i} U_i(\pi_i,\pi_{-i}) \\
&= \text{argmax}_{\pi_i} U_i^L(\pi_i)
\\
&= \text{\normalfont argmax}_{\pi_i} \bE_{\pi_i}[\sum_t \gamma^t R_i (s_t)] \\
&=\pi_i^*
\end{align*}
\end{proof}\fi

We can also consider the optimal strategy for the opposite case, if the human's utility is weighted entirely to the deployment phase. In this case, there is no incentive to be truthful---a rational human would act to match the AI's policy with their own expert policy. If a policy causes the AI's posterior reward function to equal the human's reward function, then it is optimal. This is possible if the human can act such that their posterior expected reward function is a the difference between (an affine transformation of) their actual reward function and everybody else's posterior expected reward function.

\begin{theorem}
For any $\pi_{-i}, \mathcal{M}$, if there exists $\pi_i$ such that $\mathcal{M}(\pi_i, \pi_{-i}) = \pi^*_i$, then $Br(\pi_{-i}, \mathcal{M}, 0) = \pi_i$. In particular, if there exists policy $\pi_i$ and real numbers $b>0,c$ such that $\bE_{\rewardprior} [R_i|\mathbf{a}_i] = b R_i + c  - \sum_{j \ne i} \bE_{P} [R_j|\mathbf{a}_j]$, then $\pi_i = Br_i(\pi_{-i}, \mathcal{M}^*, 0)$.
\end{theorem}
\iffalse\begin{proof}
Suppose that $\bE_{\rewardprior} [R_i|\mathbf{a}_i] = b R_i + c  - \sum_{j \ne i} \bE_{P} [R_j|\mathbf{a}_j]$ for some $b>0, c \in \bR$. Then $b R_i + c  = \sum_{j} \bE_{P} [R_j|\mathbf{a}]$. From theorem \ref{thm:deployment}, the deployment policy is optimal for reward $ \sum_{j} \bE_{P} [R_j|\mathbf{a}]$. Since optimal policy is invariant to affine transformation, the deployment policy is also optimal for $R_i$.
\end{proof}\fi


Now we consider strategies when there is weight on both the learning and deployment phases. As more weight is placed on the learning phase relative to the deployment phase, the learning utility of optimal policy weakly increases and the deployment utility of the optimal policy weakly decreases. 
\begin{proposition} \label{prop:phases}
Suppose $\alpha > \alpha'$. For any profile of policies $\pi_{-i}$, let $\pi_i = Br_i(\pi_{-i},\alpha)$ and $\pi'_i = Br_i(\pi_{-i},\alpha')$. Then $U^L_i(\pi_i) \ge U^L_i(\pi'_i)$ and $ U^D_i(\pi', \pi_{-i}) \ge U^D_i(\pi, \pi_{-i})$.
\end{proposition}
\iffalse\begin{proof}
Since $\pi_i = Br_i(\pi_{-i},\alpha)$ and $\pi'_i = Br_i(\pi_{-i},\alpha')$, neither policy can strictly dominate the other policy in both phases. Given that \[\alpha U^L_i(\pi_i) + (1-\alpha)U^D_i(\pi_i) \ge \alpha U^L_i(\pi'_i) + (1-\alpha)U^D_i(\pi'_i)\] and
\[\alpha' U^L_i(\pi'_i) + (1-\alpha')U^D_i(\pi'_i) \ge \alpha' U^L_i(\pi_i) + (1-\alpha')U^D_i(\pi_i),\] we have \[(\alpha-\alpha') (U^L_i(\pi_i)-  U^L_i(\pi'_i))- (\alpha-\alpha') (U^D_i(\pi_i)- U^D_i(\pi'_i)) \ge 0.\] Since $\alpha - \alpha' > 0$, this implies that $U^L_i(\pi_i) \ge U^L_i(\pi'_i)$ and $ U^D_i(\pi', \pi_{-i}) \ge U^D_i(\pi, \pi_{-i})$.

\end{proof}\fi

We can show that for sufficiently large $\alpha$, which can be less than one in the case of finite number of policies the expert policy is optimal.
\begin{theorem}
If \begin{equation}
    \frac{\alpha}{1-\alpha} > \frac{V(\pi^*_i,R_i) - \min_\pi V(\pi,R_i)}{V(\pi^*_i,R_i) - \max_{\pi \ne \pi^*} V(\pi,R_i)},
\end{equation} then $\pi^*$ is optimal. \end{theorem}

Hence, inverse reinforcement learning yields a natural truthful mechanism. This yields a tradeoff: as $\alpha$ increases, we can expect the fidelity of demonstrations to increase; however, increasing $\alpha$ also would mean that the AI has less of an impact to relative to the demonstration. On either end of the spectrum, an impotent AI would yield completely truthful demonstrations; a powerful AI or the lack of direct consequences for actions would cause strategic behavior from humans.  


\subsubsection{Expected Externalities} Taking inspiration from mechanism design literature \cite{d1979incentives}, we analyze the expected externality of dishonest policies.
\begin{definition}
The expected externality of policy $\pi_i$ is defined as \begin{equation}
    Ex(\pi_i)=\sum_{j \ne i} \bE_P [ U_j^D(\pi_i,\pi^*_{-i},\mathcal{M}^*)] - \sum_{j \ne i} \bE_P [U_j^D(\pi^*_i,\pi^*_{-i},\mathcal{M}^*)].
\end{equation}
\end{definition}

This is the total amount utility lost by all humans except human $i$, given that human $i$ uses policy $\pi_i$ as opposed to the expert policy. A negative value of the expected externality, for example, represents that the other humans are worse off as a whole. We can measure the impact of dishonest policies not just on social welfare, but also on the effect of dishonest policies on other participants. 

Several well-known mechanisms in mechanism design enforce honesty by requiring that a human pays for the externalities that they cause other agents. In the absence transfers, which require a pseudo-linear utility function, we instead impose the cost of misrepresentation in the learning phase. Relative to the expert policy, for any dishonest policy, if the utility lost in the learning phase is greater than the externalities caused in the deployment phase, than that policy is suboptimal.

\begin{theorem}
If 
\begin{equation}
    \alpha(U^L_i(\pi^*_i) - U^L_i(\pi_i)) \ge (1-\alpha)(-Ex(\pi_i))
\end{equation} for dishonest $\pi_i$, then $\pi_i$ is suboptimal to the expert policy.
\end{theorem}
\iffalse\begin{proof}
For dishonest $\pi_i$, 
\[\bE[\sum_{j} U_j(\pi^*_i,\pi^*_{-i})] > \bE[\sum_{j} U_j(\pi_i,\pi^*_{-i})].\] Expanding out the terms of utility, \[\bE[\sum_{j\ne i} U_j^D(\pi_i^*,\pi^*_{-i})] - \bE[\sum_{j\ne i} U_j^D(\pi_i,\pi^*_{-i})] > \bE[U_i^D(\pi_i,\pi^*_{-i})] - \bE[\sum_{j\ne i} U_i^D(\pi_i^*,\pi^*_{-i})].\] 
Thus, \[\bE U(\pi^*_i, \pi^*_i) = \alpha U^L(\pi^*_i) + (1-\alpha )\bE U^D(\pi^*_i, \pi^*_{-i})\] \\ \[>  \alpha U^L(\pi_i) + (1-\alpha )\bE U^D(\pi_i, \pi^*_{-i})  = \bE U(\pi_i, \pi^*_i)\]
\end{proof}\fi

\begin{corollary}
If \[\frac{\alpha}{1-\alpha} \ge \max_{i, \text{ \normalfont Dishonest } \pi} \frac{-Ex(\pi_i)}{U^L_i(\pi^*) - U^L_i(\pi)},\] then optimal solution is honest.  
\end{corollary}

This result implies that, if we know the set of dishonest strategies with greater deployment phase utility than the expert strategy, we can appropriate weight the learning phase to disincentivize dishonest behavior. 

\begin{remark}
For sufficiently large $\alpha$, the optimal solution for that $\alpha$ is not dishonest. In particular, if the space of policies is finite, then there exists $\alpha < 1$ that accomplishes this. 
\end{remark}

Even in cases where the optimal policy is dishonest, the relative weighting on the two phases affects the severity of the policy. 

\begin{proposition} \label{prop:deploy}
If $\pi_i$ is dishonest, then \begin{equation}
    U_i^D(\pi_i,\pi^*_{-i}) -  U_i^D(\pi^*_i,\pi^*_{-i}) < -Ex(\pi_i).
\end{equation}
The negative expected externality of dishonest strategy $\pi_i$ is lower bounded by increase in deployment utility of the agent. 
\end{proposition}
\iffalse\begin{proof}
If $\pi_i$ is dishonest, then \[\bE[\sum_{j} U_j^D(\pi^*_i,\pi^*_{-i})] > \bE[\sum_{j} U_j^D(\pi_i,\pi^*_{-i})].\] Simple algebraic manipulation shows that \[U_i^D(\pi_i,\pi^*_{-i}) -  U_i^D(\pi^*_i,\pi^*_{-i}) < -(\sum_{j \ne i} \bE U_j^D(\pi^*_i,\pi^*_{-i})] - \bE \sum_{j \ne i} U_j^D(\pi_i,\pi^*_{-i})]).\]
\end{proof}\fi

We combine the propositions \ref{prop:phases} and \ref{prop:deploy} to yield a result regarding the externalities of optimal dishonest policies. Weighting the learning phase less causes an incentive for the human to deviate more from the expert policy, resulting in greater negative externalities on the other humans.

\begin{remark}
Dishonest policies that are optimal for a given $\alpha$ must have negative externalities of at least a certain magnitude, and decreasing $\alpha$ increases the magnitude of this bound.
\end{remark}

\textcolor{blue}{\subsection{Connections to Voting Theory if Space Permits}}

